Vector Quantized Image-to-Image Translation

Current image-to-image translation methods formulate the task with conditional generation models, leading to learning only the recolorization or regional changes as being constrained by the rich structural information provided by the conditional contexts. In this work, we propose introducing the vector quantization technique into the image-to-image translation framework. The vector quantized content representation can facilitate not only the translation, but also the unconditional distribution shared among different domains. Meanwhile, along with the disentangled style representation, the proposed method further enables the capability of image extension with flexibility in both intra- and inter-domains. Qualitative and quantitative experiments demonstrate that our framework achieves comparable performance to the state-of-the-art image-to-image translation and image extension methods. Compared to methods for individual tasks, the proposed method, as a unified framework, unleashes applications combining image-to-image translation, unconditional generation, and image extension altogether. For example, it provides style variability for image generation and extension, and equips image-to-image translation with further extension capabilities.

==> tex/fig-afhq-extend.tex <==
\begin{figure}[t]
% \centering
\setlength\tabcolsep{1.5pt} % default value: 6pt
\begin{tabular}{c:ccc}
Input & Completion & + Inter-I2I & + Intra-I2I \\


%\multicolumn{2}{c}{inter translation} & intra translation \\

% cat2dog
\includegraphics[height=.49\linewidth]{images/fig8_quarter.png} &
\includegraphics[height=.49\linewidth]{images/fig8_extend.png} &
\includegraphics[height=.49\linewidth]{images/fig8_inter_trans.png} &
\includegraphics[height=.49\linewidth]{images/fig8_intra_trans.png}
\\

\end{tabular}
%\vspace{-3mm}
\caption{\textbf{Image Completion and Translation.} 
% We perform the image completion 
Given a quarter of an image from AFHQ~\cite{choi2020stargan} dataset as the input, we perform the image completion as well as inter- and intra-domain translations. Results show that, 
% translation and completion given the quarter image from AFHQ~\cite{choi2020stargan} dataset. 
our VQ-I2I is able to not only learn the joint content distribution of cats and dogs thus achieving reasonable completion but also support the diverse translation via the design of disentanglement.}
%\vspace{-3mm}
\label{fig:afhq-completion}
\end{figure}

==> tex/fig-pair.tex <==
\begin{figure}[t]
% \centering
\setlength\tabcolsep{1.5pt}

\begin{center}
%\vspace{-1em}

\begin{tabular}{c:ccc}
Input & Ours & Pix2pix & BicycleGAN \\
\includegraphics[width=.24\linewidth]{images/fig5_input_col.png} & 
\includegraphics[width=.24\linewidth]{images/fig5_ours.png} & 
\includegraphics[width=.24\linewidth]{images/fig5_pix2pix.png} & 
\includegraphics[width=.24\linewidth]{images/fig5_bicyclegan.png} \\
\end{tabular}
%\vspace{-1mm}
\caption{\textbf{Translation on Paired Cityscapes Dataset.} 
Our approach is able to handle training with paired data. The left column shows the semantic segmentation of street scenes, and the other columns show the corresponding generated scenes by various models which are trained on paired data.
}
\label{fig:visual-pair}
%\vspace{1mm}



\end{center}%



\end{figure}
